Energy-Based Models for Functional Data using Path Measure Tilting

Energy-Based Models (EBMs) have proven to be a highly effective approach for modelling densities on finite-dimensional spaces. Their ability to incorporate domain-specific choices and constraints into the structure of the model through composition make EBMs an appealing candidate for applications in physics, biology and computer vision and various other fields. Recently, Energy-Based Processes (EBP) for modelling stochastic processes was proposed for \textit{unconditional} exchangeable data (e.g., point clouds). In this work, we present a novel subclass of EBPs, called $\mathcal{F}$-EBM for \textit{conditional} exchangeable data, which is able to learn distributions of functions (such as curves or surfaces) from functional samples evaluated at finitely many points. Two unique challenges arise in the functional context. Firstly, training data is often not evaluated along a fixed set of points. Secondly, steps must be taken to control the behaviour of the model between evaluation points, to mitigate overfitting. The proposed model is an energy based model on function space that is decomposed spectrally, where a Gaussian Process path measure is used to reweight the distribution to capture smoothness properties of the underlying process being modelled. The resulting model has the ability to utilize irregularly sampled training data and can output predictions at any resolution, providing an effective approach to up-scaling functional data. We demonstrate the efficacy of our proposed approach for modelling a range of datasets, including data collected from Standard and Poor's 500 (S\&P) and UK National grid.

==> remove_paragraphs.tex <==
\begin{comment}
Since we are interested in the performance of the model when interpolating between points, we would preferably like to compute the difference between the inferred function and the underlying ``true'' function. However, this is not possible as the underlying ``function'' is usually unknown to us except in synthetic settings. Thus, to evaluate both the fidelity and usefulness of the model we purposefully obfuscate the function by removing a portion of evaluations, the inferred function is then evaluated at these points and compared against its true values. Given a $p \in (0,1)$, we consider three methods for removing a portion of $1-p$ from $(X, Y)$ to create $( \tilde{X}, \tilde{Y})$. We also write the removed sampled points as $\tilde{X}^c$ defined such that $\tilde{X} \cup \tilde{X}^c = X$ (and similarly for $\tilde{Y}^c$).The sampled points (and its values) that are discarded were chosen either uniformly without replacement, removed sampled points that were in the middle, or down-sampled the sampled points (see Figure \ref{fig:missing_setup}). 

For each desideratum, we determine if our proposed is successful by: 
\begin{enumerate}
    \item The \textit{diversity} of the samples can be assessed qualitatively by applying dimensionality reduction methods (such as t-SNE \citep{van2008visualizing} and PCA \citep{bryant1995principal}) on both the original data and the generated samples to $2$-d space. Visually, we should expect the distribution of the embeddings of both the data and model samples to be close (i.e., there is high overlap). 
    \item The \textit{fidelity} of the model can be evaluated by examining samples from the conditional distribution $p_\theta(f | \tilde{Y}; \tilde{X})$ where $\tilde{Y}$ is some obfuscated version  of the original representation $Y$. We are interested in how in close the generated functions match the original statistics of the data. To this end, we study how difference between the sample autocorrelation $\tilde{r}(\cdot)$ of the expected function $\mathbb{E}_{p_\theta(f|\tilde{Y}; \tilde{X})}[f]$ and the ``true'' sample autocorrelation $r(\cdot)$ of the original data $Y$. The difference is computed as the sum of squared error, i.e., we report $\sum_{i=1}^{n=1}(\tilde{r}(i) - r(i))^2$.
    \item Similarly, as before, we evaluate the \textit{usefulness} by studying the conditional distribution $p_\theta(f |\tilde{Y}; \tilde{X})$  where $\tilde{Y}$ is some obfuscated version  of the original representation $Y$. In this case, we are interested in the inferred functions ability to interpolate between evaluated points which we measure by computing the squared error between the actual function values and the expected function values on removed evaluation points. More precisely, we report $\sum_{(x_i,y_i) \in (\tilde{X}^c, \tilde{Y}^c)} (\mathbb{E}[f(x)] - y_i)^2$ which is averaged over the evaluation set.
\end{enumerate}
For the case that $Y$ is binary, a Bernoulli likelihood can used
\begin{align*}
    L(Y, f ; X) &:= \sum_{n=1}^M \big [y_m\log  \left (\sigma\left (f(x_n)\right) \right ) \\
                &+ (1-y_m)\log(1-\sigma(f(x_m)))\big ],
\end{align*}
where $\sigma$ is a suitable transformation (e.g., sigmoid function).
\end{comment}
